SMORE: Score Models for Offline Goal-Conditioned Reinforcement Learning

Offline Goal-Conditioned Reinforcement Learning (GCRL) is tasked with learning to achieve multiple goals in an environment purely from offline datasets using sparse reward functions. Offline GCRL is pivotal for developing generalist agents capable of leveraging pre-existing datasets to learn diverse and reusable skills without hand-engineering reward functions. However, contemporary approaches to GCRL based on supervised learning and contrastive learning are often suboptimal in the offline setting. An alternative perspective on GCRL optimizes for occupancy matching, but necessitates learning a discriminator, which subsequently serves as a pseudo-reward for downstream RL. Inaccuracies in the learned discriminator can cascade, negatively influencing the resulting policy. We present a novel approach to GCRL under a new lens of mixture-distribution matching, leading to our discriminator-free method: SMORe. The key insight is combining the occupancy matching perspective of GCRL with a convex dual formulation to derive a learning objective that can better leverage suboptimal offline data. SMORe learns scores or unnormalized densities representing the importance of taking an action at a state for reaching a particular goal. SMORe is principled and our extensive experiments on the fully offline GCRL benchmark composed of robot manipulation and locomotion tasks, including high-dimensional observations, show that SMORe can outperform state-of-the-art baselines by a significant margin.

==> old_connection_to_contrastive_learning.tex <==

\subsection{Connection to contrastive learning}
\label{sec:scogo_contrastive_connection}

To bridge the connection to contrastive RL and devise a stable learning algorithm we consider the Pearson $\chi^2$ divergence. Pearson $\chi^2$ divergence has been found to lead to distribution matching objectives that are stable to train as a result of a smooth quadratic generator function $f$~\citep{garg2021iq,al2023ls,sikchi2023dual}. \hs{missing gamma, transition from dataset} Instantiating with Pearson $\chi^2$ Divergence, our dual formulation \scogo simplifies to the following objective:
\begin{multline}
\label{eq:contrastive_scogo}
   \max_{\pi_g}\min_{S}  \color{purple}\overbrace{\color{black} \beta (1-\gamma)\E{d^O,\pi_g}{S(s,\pi_g(s),g)} +\beta \E{s,a,g\sim q,s'\sim p(\cdot|s,a)} { S(s',\pi_g(s'),g )}}^{\text{Decrease score at transitions under current policy $\pi_g$}}\\
        -\color{teal}\underbrace{\color{black}\beta \E{s,a,g\sim q}{S(s,a,g)}}_{\text{Increase score at the proposed goal transition distribution}}\color{black}+0.25\color{brown}\underbrace{\color{black}\E{s,a,g\sim d_\text{mix}^{Q,O}}{( S(s',\pi_g(s'),g )-S(s,a,g))^2} }_{\text{Bellman consistency}}
\end{multline}

\begin{wrapfigure}{R}{0.45\textwidth}
\vskip -25pt
\centering
\begin{minipage}[t]{.45\textwidth}
\begin{algorithm}[H]
    \small
        \caption{SMORe}
    \label{alg:ALG1}
    \begin{algorithmic}[1]
    \State Init $S_\phi$, $M_\psi$, and $\pi_\theta$\newline    
    \State Let $d^O = \{(s, a, s', g) \}$: data from offline replay buffer. $q(s,a,g) = \{(s, a, s', g) \}$ be goal-transition distribution\newline
    \For {step $t$ in \{1...N\}}
        \State Train $S_\phi$ using $\mathcal{L}(\phi)$ from Eq.~\ref{eq:practical_s_update}\newline
        \State Train $M_\theta$ using $\mathcal{J}(\psi)$ from  Eq.~\ref{eq:practical_m_update} \newline 
        \State Update $\pi_\psi$ via Eq.~\ref{eq:practical_pi_update} \newline
    \EndFor
    \end{algorithmic}
\end{algorithm}
\end{minipage}
% \vskip-10pt
\end{wrapfigure}
Equation~\ref{eq:contrastive_scogo} makes the connection between \scogo and contrastive RL more obvious while providing us with a surprising insight.  Contrastive RL~\citep{eysenbach2020c} maximizes the $Q$-function at s,a,g for goals $g$  that are achieved in the observed trajectory while minimizing the score at randomly sampled $g$. In contrast, our method suggests a different contrastive procedure, maximizing the score at goal-transition distribution and minimizing the score at the offline data distribution under current policy while maintaining Bellman consistency. Instantiating with KL divergence results in an objective with similar intuition while resembling an infoNCE~\citep{oord2018representation} objective. The weighting for the additional Bellman consistency term is suggested by theory to be 0.25 relative to the weighting for the contrastive losses in order to devise a principled GCRL method. It is important to note that $S$-function is not grounded to any rewards and does not serve to be a probability density of reaching goals but is rather a score function learned via \textit{a Bellman-consistent contrastive learning procedure}.

==> relation_between_mixture_and_vanilla_divergence.tex <==

\subsection{Relation between divergence and training objective}

\todoah{Tentative}
for any policy $\pi$ and any function $S$ over state-action-goal, we have,
\begin{align}
    D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O) & = D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O) \\
     & - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d^{\pi}  - d^{pi} \rangle \nonumber
\end{align}
This follows from the fact that $d^\pi$ is an occupancy measure, which implies that 
$ (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d^{\pi}  - d^{\pi} = 0$.

% Let consider d any function over state-action-goal, we have: 
% \begin{align}
%     & D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)\\
%     & =  D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d \rangle \\
%      & + D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)  - D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O)\\
%      & + \langle S, \gamma P^{\pi}^\top (d^\pi - d) \rangle \\
%      & \leq D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d \rangle \\
%      & +  \left |  D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)  - D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) \right | \\
%      & +  \left | \langle S, \gamma P^{\pi}^\top (d^\pi - d) \rangle \right |
% \end{align}
% The latter inequality holds for any $d$, so we can take the minimum over $d$ in the right-hand-side. we obtain: 

% \begin{align}
%     & D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)\\
%      & \leq \min_d D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d \rangle \\
%      & +  \min_d \left |  D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)  - D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) \right | \\
%      & +  \min_d \left | \langle S, \gamma P^{\pi}^\top (d^\pi - d) \rangle \right | \\
%      & = \min_d D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d \rangle
% \end{align}
% The latter egality comes from the fact that minimum is acheived at $d = d^\pi$. We can conclude then that
% \begin{align}
% & D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)\\
%      & \leq \max_S \min_d D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d \rangle
% \end{align}

% Similarly, we can show that

% \begin{align}
%     & D_f( \beta d^\pi + (1- \beta) d^O\| \beta q + (1- \beta) d^O)\\
%      & \geq - \max_S \min_d D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) - \langle S, (1 - \gamma) d_0 \pi + \gamma P^{\pi}^\top d \rangle
% \end{align}




\subsection{Relation between $D_f( d \| q)$ and $D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O)$ }
\begin{align}
    f \left( \frac{\beta d + (1- \beta) d^O}{\beta q + (1- \beta) d^O} \right) &= f \left( \frac{\beta d }{\beta q + (1- \beta) d^O} + \frac{(1- \beta) d^O}{\beta q + (1- \beta) d^O} \right)  \\
    & = f \left( \frac{\beta q }{\beta q + (1- \beta) d^O} \left(\frac{d}{q}\right) + \frac{(1- \beta) d^O}{\beta q + (1- \beta) d^O} \times  1 \right) \\
    & \leq \frac{\beta q }{\beta q + (1- \beta) d^O}  f\left(\frac{d}{q}\right) + \frac{(1- \beta) d^O}{\beta q + (1- \beta) d^O} f(1) \\
    & = \frac{\beta q }{\beta q + (1- \beta) d^O}  f\left(\frac{d}{q}\right)
\end{align}
the two last steps follow respectively from the fact that $f$ is convex and $f(1) = 0$.
Therefore,
\begin{align}
    D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) & = \sum (\beta q + (1- \beta) d^O) f \left( \frac{\beta d + (1- \beta) d^O}{\beta q + (1- \beta) d^O} \right) \\
    & \leq \sum (\beta q + (1- \beta) d^O) \frac{\beta q }{\beta q + (1- \beta) d^O}  f\left(\frac{d}{q}\right) \\
    & = \beta \sum q f\left(\frac{d}{q}\right) \\
    & = \beta D_f(d \| q)
\end{align}
Hence 
\begin{equation}
    D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O)  \leq \beta D_f(d \| q)
\end{equation}
\todoah{This actually can be seen as a consequence of the Data Processing inequality}

We have equality for the total variation: 
\begin{align}
    D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) 
    & = \frac{1}{2}\sum (\beta q + (1- \beta) d^O) \left | \frac{\beta d + (1- \beta) d^O}{\beta q + (1- \beta) d^O} - 1 \right | \\
    & = \frac{1}{2} \sum | (\beta d + (1- \beta) d^O) - (\beta q + (1- \beta) d^O) | \\
    & = \frac{1}{2} \beta \sum |q  - d| = \beta D_f(d \| q)
\end{align}

% For Pearson: 
% \begin{align}
%     D_f( \beta d + (1- \beta) d^O\| \beta q + (1- \beta) d^O) 
%     & = \sum (\beta q + (1- \beta) d^O) \left ( \frac{\beta d + (1- \beta) d^O}{\beta q + (1- \beta) d^O} - 1 \right )^2 \\
%     & = \sum  \beta^2 (d - q)^2 \frac{1}{(\beta q + (1- \beta) d^O)} \\
% \end{align}

